It is undecidable if two regular tree languages can be separated by a deterministic tree-walking automaton

The following problem is shown undecidable: given regular languages L,K of finite trees, decide if there exists a deterministic tree-walking automaton which accepts all trees in L and rejects all trees in K. The proof uses a technique of Kopczy\'nski from LICS 2016.

==> smieci.tex <==

\subsection{A sufficient condition for undecidable separability}
The ``certain properties'' of a class $\Ll$ that we mentioned above are that: a) the class is a pseudo-variety of tree languages; b) 

\subsection{Pseudovariety of tree languages} Let $\Sigma, \Gamma$ be ranked alphabets. 
Define a \emph{tree homomorphism} to be a function
\begin{align*}
	h : \trees   \Sigma \to \trees \Gamma
\end{align*}
which replaces each letter $a \in \Sigma$ with a term over $\Gamma$ of same arity that depends only on $a$. In other words, for every $a \in \Sigma$ of arity $n$ there exists some $t \in \trees_n \Gamma$ such that
\begin{align*}
	h(a(t_1,\ldots,t_n)) = t(h(t_1),\ldots,h(t_n)) \qquad \mbox{for all $t_1,\ldots,t_n \in \trees \Sigma$}.
\end{align*}
We underline once again that our notion of terms allows each argument to be used only once. Typically tree homomorphisms can duplicate subtrees, and the notion of tree homomorphism that we use is called a \emph{linear tree homomorphism}, see e.g.~\cite{DBLP:books/others/tree1984}.

\begin{definition}\label{def:pseudovariety}
	A class of tree languages is called a \emph{pseudovariety} if it has the following three closure properties:
	\begin{itemize}
		\item {\bf Boolean }It is closed under union, intersection and complementation;
		\item {\bf Quotients.} For every $t \in \trees_1 \Sigma$, if the class contains $L \subseteq \trees \Sigma$, then it also contains
		\begin{align*}
			\set{s \in \trees \Sigma: t(s) \in L}
		\end{align*}
		\item {\bf Homomorphisms.} For every tree homomorphism $h : \trees \Sigma \to \trees \Gamma$, if the class contains $L \subseteq \trees \Gamma$, then it also contains
		\begin{align*}
			 \set{s \in \trees \Sigma : h(s) \in L}
		\end{align*}
	\end{itemize}
\end{definition}

\begin{myexample}
	We claim that the class of tree languages recognised by deterministic tree-walking automata forms a pseudovariety.  Closure under intersection is immediate: we first run the automaton for the first language, and then we run the automaton for the second language. Closure under complementation is more subtle, because a deterministic tree-walking automaton might reject by entering an infinite loop. As mentioned above, in~\cite{} it is shown that deterministic tree-walking automata can be complemented, because every deterministic tree-walking automaton can be converted (even in polynomial time) into one which never enters an infinite loop. 
	
	We are left with quotients and homomorphisms. We only do the homomorphisms, with quotients being done the same way. For inverse images under homomorphisms, we need to show that if 
	\begin{align*}
		h : \trees \Sigma \to \trees \Gamma
	\end{align*} is a tree homomorphism, and $\Aa$ is a deterministic tree-walking automaton over $\Gamma$, then there is a deterministic tree-walking automaton over $\Sigma$ which accepts a tree $t \in \trees \Sigma$ if and only if $\Aa$ accepts $h(t)$.
\end{myexample}



\newcommand{\autclass}	{\mathsf{aut}}
Define $\autclass \Ll$ to be those automata $\Aa$ such that every state is accessible and  for every choice of accepting states, the recognised language is in $\Ll$.  For an automaton $\Aa$ with states $Q$ and input alphabet $\Sigma$, and a term $t \in \trees_n \Sigma$, define 
\begin{align*}
	t^\Aa : Q^n \to Q
\end{align*}
to be the state transformation defined in the natural way.


\begin{lemma}\label{lem:undecidable-general}
Let $\Ll$ be a pseudovariety of tree languages such that:
\begin{enumerate}
	\item if $\Aa \in \autclass \Ll$ has input alphabet $\Sigma$ then there is a term $t \in \trees_2 \Sigma$ such that the following two ternarny terms induce the same state transformation:
	\begin{align*}
		t(x,t(y,z)) \qquad t(t(x,y),z)
	\end{align*}
	% \item there is no language from $\Ll$ that separates the following two languages over alphabet
	% \begin{align*}
	% 	\Sigma = \set{\underbrace{a}_{\text{rank 2}}, \underbrace{b,c}_{\text{rank 0}}}
	% \end{align*}
	% \begin{enumerate}
	% 	\item there are exactly three leaves with label $c$, and the $c$-branching structure is like this:
	% 	\begin{center}
	% 		(TODO picture)
	% 	\end{center}
	% 	\item there are exactly three leaves with label $c$, and the $c$-branching structure is like this:
	% 	\begin{center}
	% 		(TODO picture)
	% 	\end{center}
	% \end{enumerate}
	\item for every $n \in \Nat$, every alphabet $\Sigma$ and symbols $a,b \in \Sigma$ of rank zero, the class $\Ll$ contains the language
	\begin{quote}
		there are at least $n$ leaves with labels in $\set{a,b}$, and among those leaves, the $n$-th one from the left has label $a$.
	\end{quote}
\end{enumerate}	
Then the following problem is undecidable:
\begin{itemize}
	\item Input: two regular tree languages;
	\item Question: can they be separated by some language from $\Ll$?
\end{itemize}
\end{lemma}

Before proving the above lemma, let us show that the class of tree languages recognised by deterministic tree-walking automata satisfies the assumptions of the above lemma, and therefore Theorem~\ref{thm:undecidable-dtwa} follows.

\begin{pr}[of Theorem~\ref{thm:undecidable-dtwa}]
\begin{enumerate}
	\item 
	\item Condition 2 is Theorem .. in~\cite{}. 
	\item Condition 3 is easily seen to be tree, the appropriate automaton does a depth-first search traversal of the tree.
\end{enumerate} 
 
 
	
\end{pr}

Before proving 
\begin{pr}
	We check that the assumptions of t
\end{pr}





\begin{pr}
	Let $\Sigma$ be the alphabet of $[G],[H]$, i.e.~this is the nonterminals in the grammar seen as rank 0 letters plus two extra letters $a,b$ of arities $2$ and $0$.
	Suppose that $L \subseteq \trees \Sigma$ is  a tree language from $\Ll$ that contains $[G]$ and is disjoint from $[H]$. 
	
	Because $\Ll$ is a pseudovariety, there is some automaton $\Aa \in  \Ll$ that recognises $L$. By condition .. in Lemma~\ref{lem:undecidable-general}, there is some
	\begin{align*}
		t \in \trees_2 \set{a,b}.
	\end{align*}
Define $t^*$ to be the smallest set of terms that contains $t$ and is closed under composing terms, i.e.
	\begin{align*}
		t \in t^* \qquad \mbox{and} \qquad t_1,t_2 \in t^* \mbox{ implies } t(t_1,t_2) \in t^*
	\end{align*}
	
	\begin{claim}\label{claim:rotation}
Every two terms in $t^*$ of the same arity define the same state transformation on $\Aa$.		
	\end{claim}
\begin{pr}
Every two binary trees with the same number of leaves can be transformed into each other using only rotations.
\end{pr}

Let $\Gamma$ be the set of nonterminals, viewed as a set of trees. Let $K \subseteq \Gamma^*$ be the regular word language obtained by applying the comb claim to $L,t$ and $\Gamma$. For every $a_1 \cdots a_n \in \Gamma^*$ and every $n$-ary term $s \in t^*$ we have
\begin{align*}
	s(a_1,\ldots,a_n) \in L \qquad \underbrace{\mbox{iff}}_{\text{Comb Lemma}} \qquad t^{[n]}(a_1,\ldots,a_n) \in L \qquad \underbrace{\mbox{iff}}_{\text{Claim~\ref{claim:rotation}}}  \qquad a_1 \cdots a_n \in K.
\end{align*}
	
	By definition of $[G]$, for every word $a_1 \cdots a_n \in \Sigma^+$ that is generated by the grammar $G$, there is some $s \in t^*$ of arity $n$ such that
	\begin{align*}
		s(a_1,\ldots,a_n) \in [G] \subseteq L.
	\end{align*}

	and therefore the above tree belongs to $L$. Because $s \in t^*$, we know that for every $s' \in t^*$ with $n$ ports we have
	\begin{align*}
		s'(a_1,\ldots,a_n) \in L.
	\end{align*}
	In particular, choose $s'$ to be a tree which looks like this:
\begin{center}
	(todo picture)
\end{center}

	such that 
	Let $\Aa$ be the automaton recognising $L$.  it belongs to $ L$. Apply Lemma .. to $\Aa$, yielding terms $t_1,t_2 \in \trees_3 \set{a,b}$. 
\end{pr}
	
	
	
	
	and let $\Sigma$ be the alphabet, i.e.~the set of terminals. A \emph{derivation} of $G$ is a tree, where binary nodes are labelled by nondeterminals and leaves are labelled by terminals. Since we use Chomsky normal form, the derivation is a binary tree. Suppose that $t$ is a tree over the alphabet $\Sigma \cup \set \blank$ and $s$ is a derivation in the grammar $G$. We say that \emph{$t$ instanciates to $s$} if one can get $s$ from $t$ by the following process:
	\begin{itemize}
		\item remove some nodes with label $a$;
		\item for each remaining node with label $a$, change its label to some nonterminal.
	\end{itemize}
	A tree $t$ might instanciate to many $s$, or none. Here is a picture of the definition:
	\begin{center}
		picture
	\end{center}
Define
\begin{align*}
	\deriv G = \set{t \in \trees(\Sigma \cup \set \blank) : \mbox{$t$ instanciates to some derivation of $G$}}.
\end{align*}
It is not difficult to see that the above is a regular tree language, e.g.~by providing a nondeterministic tree automaton and then determinising it. Therefore, Theorem~\ref{thm} follows immediately from the undecidability in~\cite{} and the following lemma.

\begin{lemma}\label{lem:}
	Let $G_1,G_2$ be grammars in Chomsky normal form. Then the following conditions are equivalent:
	\begin{enumerate}
		\item The (word) languages of $G_1,G_2$ can be separated by a regular word language;
		\item The (tree) languages $\deriv G_1$ and $\deriv G_2$ can be separated by a deterministic tree-walking automaton.
	\end{enumerate}
\end{lemma}

The implication from 1 to 2 is straightforward -- if a $L \subseteq \Sigma^*$ is a regular word language, then one can easily compute a deterministic tree-walking automaton which accepts a tree if and only if the sequence of leaf labels, when read from left to right, formas a word in $L$. Therefore, the rest of this paper is devoted to the converse implication.


\input{twa}
\begin{lemma}\label{lem:}
	Let $\Aa$ be a deterministic tree-walking automaton. There exist 
	\begin{align*}
		t_0 \in \trees_0 \set{a} \qquad 		t_1 \in \trees_1 \set{a} \qquad 		t_2 \in \trees_2 \set{a} \qquad 
	\end{align*}
	and a function 
	\begin{align*}
		\tau : Q \to \set{\text{left,stay, root, right}}
	\end{align*}
	
\end{lemma}



==> twa.tex <==
\newcommand{\lero}[2]
{	\begin{array}{cc} {#2} \\
{#1}	\includegraphics[scale=0.3]{pics/left-root}  \ 
	\end{array}}

\newcommand{\role}[2]
{	\begin{array}{cc} {#1} \\
{#2}	\includegraphics[scale=0.3]{pics/root-left}  \ 
	\end{array}}


\newcommand{\riro}[2]
{	\begin{array}{cc} {#2} \\
	\includegraphics[scale=0.3]{pics/right-root} {#1} \ 
	\end{array}}

\newcommand{\rori}[2]
{	\begin{array}{cc} {#1} \\
	\includegraphics[scale=0.3]{pics/root-right} {#2}  \ 
	\end{array}}

\newcommand{\rile}[2]
{	\begin{array}{cc}  \\
	{#2} \includegraphics[scale=0.3]{pics/right-left} {#1} \ 
	\end{array}}

\newcommand{\leri}[2]
{	\begin{array}{cc}  \\
	{#1} \includegraphics[scale=0.3]{pics/left-right} {#2}  \ 
	\end{array}}


\begin{lemma}\label{lem:}
	Let $\Aa$ be a deterministic tree-walking automaton whose input alphabet includes a letter $a$. There exist 
	\begin{align*}
		t_0 \in \trees_0 \set{a} \qquad 		t_1 \in \trees_1 \set{a} \qquad 		t_2 \in \trees_2 \set{a} \qquad 
	\end{align*}
	such that for every $s$ which is a composition of $\set{t_0,t_1,t_2}$, if $s$ has $i \in \set{0,1,2}$ ports then $s$ has the same behaviour as $t_i$ with respect to $\Aa$.	
\end{lemma}




Let us fix $t_0,t_1,t_2$ as in the above lemma. For a tree $s \in \trees_0 \Sigma$, define 
\begin{align*}
	[s] \in \trees_0 (\Sigma \cup \set a)
\end{align*}
by replacing every binary node with $t_0$ and replacing every leaf with label $b \in \Sigma$ by $t_0(a)$.
	

\begin{align*}
 	\lero p q \role p q \riro p q  \rori p q \rile p q \leri p q
\end{align*}


\begin{definition}\label{def:}
	We say that a state $p$ has \emph{upward behavior} if 
	\begin{align*}
		\lero p p \qquad \mbox{and} \qquad \riro p p 
	\end{align*}
	We say that a pair of states $(p,q)$ has \emph{left-to-right search behavior} if
	\begin{align*}
		\riro p p \qquad \mbox{and} \qquad \leri p q \qquad \mbox{and} \qquad    \role q q
	\end{align*}
	We say that a pair of states $(p,q)$ has \emph{right-to-left search behavior} if
	\begin{align*}
		\lero p p \qquad \mbox{and} \qquad \rile p q \qquad \mbox{and} \qquad    \rori q q
	\end{align*}
	
\end{definition}



\begin{lemma}\label{lem:}
	Let $\Aa$ be a deterministic tree-walking automaton. There exists
	\begin{align*}
 		t_1 \in \trees_1 \set{a} \qquad 		t_2 \in \trees_2 \set{a} \qquad 
	\end{align*}
	
	such that if $p$ is a $t$-return state, then 
\end{lemma}

